GLIN: A (G)eneric (L)earned (In)dexing Mechanism for Complex Geometries

Although spatial indexes shorten the query response time, they rely on complex tree structures to narrow down the search space. Such structures in turn yield additional storage overhead and take a toll on index maintenance. Recently, there have been a flurry of efforts attempting to leverage Machine-Learning (ML) models to simplify the index structures. However, existing geospatial indexes can only index point data rather than complex geometries such as polygons and trajectories that are widely available in geospatial data. As a result, they cannot efficiently and correctly answer geometry relationship queries. This paper introduces GLIN, an indexing mechanism for spatial relationship queries on complex geometries. To achieve that, GLIN transforms geometries to Z-address intervals, and then harnesses an existing order-preserving learned index to model the cumulative distribution function between these intervals and the record positions. The lightweight learned index greatly reduces indexing overhead and provides faster or comparable query latency. Most importantly, GLIN augments spatial query windows to support queries exactly for common spatial relationships. Our experiments on real-world and synthetic datasets show that GLIN has 80\%-90\% lower storage overhead than Quad-Tree and 60% - 80% than R-tree and 30% - 70% faster query on medium selectivity. Moreover, GLIN's maintenance throughput is 1.5 times higher on insertion and 3 - 5 times higher on deletion.

==> maintenance.tex <==
\section{Index Maintenance}\label{sec:maintenance}
{\indextitle} will update its index structure when the underlying data receives insertion and deletion.

For insertion, {\indextitle} takes as input a geometry key and inserts it to the index. To insert a new record, {\indextitle} first obtains the $Zmin$ address for the geometry key in this record using the approach described in Section~\ref{sec:zaddress}, then inserts the record to the base index.  Once {\indextitle} puts the new record in a leaf node, it expands the MBR of the leaf node to include the new geometry.

For deletion, the input is a geometry key and {\indextitle} deletes records that have the same key. Similar to the insertion, the first step to delete a geometry key is to get the $Zmin$ address of this geometry. It is possible that several different geometries share the same  $Zmin$ addresses. In that case, {\indextitle} only erases records that have the same geometry key. The MBR of the involved leaf node will not be shrunk after the deletion because it requires a scan of all records in this leaf node to get the latest MBR. However, this does not affect the correctness of {\indextitle} as the out-of-date MBR only introduces more false positives instead of true negatives.


%Insertion and deletion into the table will triggler the maintaining the index. It is necssary to secure that the database
%\textbf{Node expanding, splitting and merging.}
%When a leaf node is close to be full (controlled by a upper density limit), {\indextitle} will expand or split this leaf node as described in ALEX~\cite{DMY+20}. 
% The expansion will create a larger array with more gaps, retrain the model and reload the records to this array. The expanded node replaces the old leaf node. The MBR will not require an update since the records remain the same in the process.
%To split a node, {\indextitle} partitions the records to new nodes, retrains the models and reloads the records.  Each new node will have a new MBR.
%When a leaf node is close to be empty (controlled by a lower density limit), {\indextitle} will merge this node with its sibling and the merged node will have a new MBR. The details of density limits and the related cost model are beyond the scope of this paper and can be found in~\cite{DMY+20}.
